A New Paradigm in Split Manufacturing: Lock the FEOL, Unlock at the BEOL

Split manufacturing was introduced as an effective countermeasure against hardware-level threats such as IP piracy, overbuilding, and insertion of hardware Trojans. Nevertheless, the security promise of split manufacturing has been challenged by various attacks, which exploit the well-known working principles of physical design tools to infer the missing BEOL interconnects. In this work, we advocate a new paradigm to enhance the security for split manufacturing. Based on Kerckhoff's principle, we protect the FEOL layout in a formal and secure manner, by embedding keys. These keys are purposefully implemented and routed through the BEOL in such a way that they become indecipherable to the state-of-the-art FEOL-centric attacks. We provide our secure physical design flow to the community. We also define the security of split manufacturing formally and provide the associated proofs. At the same time, our technique is competitive with current schemes in terms of layout overhead, especially for practical, large-scale designs (ITC'99 benchmarks).

==> cameraready/method.tex <==
\section{Methodology}

In this section, we outline our strategy to generate the layout with industry standard EDA tools, namely, Synopsys Design Compiler (DC), Synopsys IC Compiler (ICC), and Cadence Innovus along with our in-house scripts. The synthesis is done using Synopsys Design compiler (DC). Note that we use GloabalFoundry's 65nm LPe technology library at slow process corner at 1.08V and 125C for implementation and analysis . The synthesized locked netlist is imported to Synopsys IC compiler (ICC) for layout generation. Next, at the placement stage the location of the TIELO/TIEHI cells are randomized. We restrict the TIELO/TIEHI cells to single fan-outs. This eliminates any inference to be made between key bits as the key net connections remain independent. In addition, we put an extra constraint to the IC compiler to prevent it from optimizing the TIELO/TIEHI cells. 
Finally, we take the design through the routing stage, and lift the key nets to the desired BEOL layers. As a proof of concept, one key net in the layout of b14\_C is shown in Fig.~\ref{fig:route}. Note that the net lifting is the most crucial step, as otherwise, the key bits would be readily available to the attacker at the FEOL. We emphasize that all our layouts are {\em DRC} and {\em LVS-clean}, and we only report the power, performance, and area number from those layouts.
   

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.8\columnwidth] {./figures/key_net_route.PNG} 
	\caption{The locked layout for b14\_C circuit. A lifted key net is shown with white. Note that the distance between the cells dissolves any proximity-induced information leakage.} 
	\label{fig:route}
\end{figure}

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.5\columnwidth] {./figures/tie_lo_cell.PNG} 
% 	\caption{Key net lifted to the BEOL.} 
% 	\label{fig:net}
% \end{figure}
